Beyond Baby Blues: The Child Penalty in Mental Health in Switzerland

This paper investigates the mental health penalty for women after childbirth in Switzerland. Leveraging insurance data, we employ a staggered difference-in-difference research design. The findings reveal a substantial mental health penalty for women following the birth of their first child. Approximately four years after childbirth, there is a one percentage point (p.p.) increase in antidepressant prescriptions, representing a 50% increase compared to pre-birth levels. This increase rises to 1.7 p.p. (a 75% increase) six years postpartum. The mental health penalty is likely not only a direct consequence of giving birth but also a consequence of the changed life circumstances and time constraints that accompany it, as the penalty is rising over time and is higher for women who are employed.

==> Kaiserschnitt_diff_diff.tex <==
no & 0.85 & 0.85 & 0.08\\
yes & 0.15 & 0.15 & 0.08\\


==> accident_diff_diff.tex <==
no & 0.85 & 0.82 & 7.46\\
yes & 0.15 & 0.18 & 7.46\\


==> accident_event_stagg_diff_men.tex <==
yes & 0.88 & 0.91 & 8.59 & 0.87 & 3.27 & 0.80 & 0.89 & 24.91\\



==> accident_event_stagg_diff_women.tex <==
no & 0.80 & 0.76 & 11.61 & 0.77 & 9.31 & 0.72 & 0.83 & 24.86\\
yes & 0.20 & 0.24 & 11.61 & 0.23 & 9.31 & 0.28 & 0.17 & 24.86\\


==> counts_event_stagg_diff_men.tex <==
N & 5749 & 20642 & 4057 & 629 & 5120\\


==> counts_event_stagg_diff_women.tex <==
N & 25120 & 83605 & 18714 & 5634 & 19486\\


==> income_subsidy_age_diff_diff.tex <==
income index & -0.52 & 0.27 & -0.54 & 0.26 & 6.08\\
subsidy & 0.19 & 0.39 & 0.19 & 0.39 & 0.79\\
age at first birth & 31.01 & 2.84 & 30.07 & 2.89 & 32.80\\

